Measuring Retrieval Complexity in Question Answering Systems

In this paper, we investigate which questions are challenging for retrieval-based Question Answering (QA). We (i) propose retrieval complexity (RC), a novel metric conditioned on the completeness of retrieved documents, which measures the difficulty of answering questions, and (ii) propose an unsupervised pipeline to measure RC given an arbitrary retrieval system. Our proposed pipeline measures RC more accurately than alternative estimators, including LLMs, on six challenging QA benchmarks. Further investigation reveals that RC scores strongly correlate with both QA performance and expert judgment across five of the six studied benchmarks, indicating that RC is an effective measure of question difficulty. Subsequent categorization of high-RC questions shows that they span a broad set of question shapes, including multi-hop, compositional, and temporal QA, indicating that RC scores can categorize a new subset of complex questions. Our system can also have a major impact on retrieval-based systems by helping to identify more challenging questions on existing datasets.

==> tables/generative_results_qa.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \textbf{Not Complex} & \textbf{Complex} \\ \midrule
CWQ & 0.703 & 0.313 \\ 
HotPotQA & 0.141 & 0.250 \\ 
Quora & 0.016 & 0.0156 \\ 
NQ & 0.594 & 0.031 \\ 
StrategyQA & 0.031 & 0.0 \\ 
musique & 0.563 & 0.0469 \\ \bottomrule
\end{tabular}
\caption{Results of complex vs not complex questions selected by the pipeline when generating an answer with a LLM.  The results have been computed in terms of partial match with the original references. Each answer has been generated using Mistral 7B.}
\label{tab:generative_results}
\end{table}

==> tables/human_annotation.tex <==
\begin{table}[]
\resizebox{1\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Dataset}   & \textbf{Accuracy} & \textbf{Correlation} \\\midrule
Natural Questions  &                   &                      \\
QuoraQP-a          &                   &                      \\
\bottomrule
\end{tabular}
}
\caption{Result for the manual evaluation in terms of Accuracy.}
\label{tab:human_correlation}
\end{table}

==> tables/search_engine.tex <==
\begin{table}[]
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Approach}        & \multicolumn{3}{c}{\textbf{Accuracy}}      \\
\textbf{}                & \textbf{NQ} & \textbf{CWQ} & \textbf{TriviaQA} \\ \midrule
Bing                   &             &              &               \\ \bottomrule
\end{tabular}
\caption{Results of commercial and industrial search engines on complex questions.}
\label{tab:search_engine_results}
\end{table}
